Source-Free Domain-Invariant Performance Prediction

Accurately estimating model performance poses a significant challenge, particularly in scenarios where the source and target domains follow different data distributions. Most existing performance prediction methods heavily rely on the source data in their estimation process, limiting their applicability in a more realistic setting where only the trained model is accessible. The few methods that do not require source data exhibit considerably inferior performance. In this work, we propose a source-free approach centred on uncertainty-based estimation, using a generative model for calibration in the absence of source data. We establish connections between our approach for unsupervised calibration and temperature scaling. We then employ a gradient-based strategy to evaluate the correctness of the calibrated predictions. Our experiments on benchmark object recognition datasets reveal that existing source-based methods fall short with limited source sample availability. Furthermore, our approach significantly outperforms the current state-of-the-art source-free and source-based methods, affirming its effectiveness in domain-invariant performance estimation.

==> sec/0_abstract.tex <==
\begin{abstract}

Accurately estimating model performance poses a significant challenge, particularly in scenarios where the source and target domains follow different data distributions. Existing performance prediction methods heavily rely on the source data in their estimation process, limiting their applicability in a more realistic setting where only the trained model is accessible. To overcome this limitation, we propose a source-free approach centred on uncertainty-based estimation, using a Gaussian Mixture Model (GMM) transformation for calibration in the absence of source data. We establish connections between our GMM-based approach for unsupervised calibration and temperature scaling.

We then employ a gradient-based strategy to evaluate the correctness of the GMM-calibrated predictions.
Our experiments on benchmark object recognition datasets show that our approach outperforms the state-of-the-art by a substantial margin, confirming its effectiveness for performance estimation in a source-free and domain-invariant setting.




%, within the softmax function. 
%which are either based on entropy thresholding or data augmentation "add citation" 
%After applying our proposed transformation to reduce prediction certainty, we introduce a gradient-based evaluation, inspired by "add citation", as a means of assessing correctness of predictions. 

%I wrote another slightly different version below. 
%TODO for Katya, please combine or change where needed

%Accurately estimating model performance poses a significant challenge in computer vision due to domain shifts between source and target datasets. Typically, existing entropy-based or augmentation-based methods "citations to COT, etc." for performance prediction rely on access to the source data in their threshold estimation or augmentation process, limiting their practical applicability when the source data is not available. In contrast, we introduce a "source-free" paradigm, where we don't need access to source data but only rely on the trained model. Our method focuses on addressing the issue of prediction overconfidence in neural networks. To mitigate this, we introduce an unsupervised calibration method using a Gaussian Mixture Model (GMM) transformation, distinct from traditional temperature scaling. We establish connections between our GMM-based approach and temperature scaling within the softmax function. After applying this transformation to reduce prediction certainty, we evaluate correctness by comparing predictions to a uniform distribution using gradient norms derived from loss backpropagation. Our experiments on benchmark datasets of .... demonstrate the superiority of our source-free domain-invariant accuracy prediction method over existing state-of-the-art techniques.
\end{abstract}

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/experiments_old.tex <==


\begin{table*}[ht]

\begin{center}
\caption{Mean Absolute Error Between Predicted and Ground Truth Accuracy for CIFAR-Corrupted. Methods are estimating the threshold based on \textbf{the Source Set}}
%\vspace{-2ex}
\label{table:layer_choice}
\scalebox{0.9}{
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\toprule
%\hline

% ToDo: Katya Left indent 

 % &\multicolumn{4}{|c|}{ Digits, MiniVGG} &\multicolumn{4}{|c|}{COCO, AlexNet}\\
 
% & \multicolumn{4}{|c|}{Size = 1000}\\
  \hline
 & gauss & shot & impls  & defoc & glass  &motion  & zoom  & snow & frost & fog & bright& contr & elast.&  pix & jpg & Mean \\\hline
 Probab &39.42 & 31.27 & 19.9 & 13.93 & 20.75 & 9.75 & 11.58 & 6.15 & 16.36 & 6.42 & 1.3 & 10.15 & 2.48 & 26.73 & 4.74 & 14.72\\ \hline 
\textbf{Bias } & 39.28 & 31.11 & 19.58 & 13.75 & 20.59 & 9.66 & 11.46 & 6.08 & 16.17 & 6.39 & 1.28 & 10.03 & 2.4 & 26.63 & 4.6 & 14.60\\ \hline
Entropy & 39.1 & 30.5 & 17.88 & 12.96 & 19.64 & 9.29 & 10.99 & 5.92 & 15.74 & 6.3 & 1.2 & 9.35 & 1.9 & 26.32 & 4.14 & 14.08 \\ \hline 
OOD loss & 40.59 & 30.96 & 5.96 & 2.26 & 10.12 & 2.84 & 2.93 & 3.83 & 15.94 & 3.34 & 0.07 & 4.7 & 4.59 & 24.65 & 3.81 & 10.43\\ \hline
  &   &   &   &   &   &   &   &   &   &   &   &   &   &  & & \\\
GT Acc &  27.67 & 34.29 & 27.08 & 53.06 & 45.68 & 65.25 & 57.98 & 74.93 & 58.7 & 73.99 & 90.7 & 53.31 & 73.41 & 41.55 & 69.7 & \\ \hline

\bottomrule
\end{tabular}
}
}
\end{center}
\vspace{-1ex}
\end{table*}



\begin{table*}[ht]

\begin{center}
\caption{Mean Absolute Error Between Predicted and Ground Truth Accuracy for CIFAR-Corrupted. \textbf{Source-Free}}
%\vspace{-2ex}
\label{table:layer_choice}
\hspace*{-11ex} \scalebox{0.9}{
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\toprule
%\hline

% ToDo: Katya Left indent 

 % &\multicolumn{4}{|c|}{ Digits, MiniVGG} &\multicolumn{4}{|c|}{COCO, AlexNet}\\
 
% & \multicolumn{4}{|c|}{Size = 1000}\\
  \hline
 & gauss & shot & impls  & defoc & glass  &motion  & zoom  & snow & frost & fog & bright& contr & elast.&  pix & jpg & Mean \\\hline
 \multicolumn{17} {|c|}{Fixed Temperature}\\  \hline 
 No Temp & 66.01 & 59.18 & 59.67 & 40.17 & 47.09 & 29.95 & 36.25 & 21.39 & 36.79 & 22.75 & 8.1 & 39.17 & 22.1 & 52.46 & 25.27 & 37.75\\ \hline
  % Newton grad & -68.05 & -61.2 & -62.35 & -41.56 & -48.58 & -31.08 & -37.5 & -22.5 & -38.07 & -23.64 & -8.42 & -40.69 & -23.09 & -54.0 & -26.24& 39.13\\ \hline
 % Energy & 68.95 & 62.4 & 64.43 & 43.28 & 50.16 & 32.29 & 38.92 & 23.14 & 38.83 & 24.33 & 8.75 & 42.58 & 24.29 & 55.25 & 27.65 & 40.34\\ \hline
  Tempr:1/2 &53.93 & 45.36 & 34.91 & 26.4 & 32.79 & 20.18 & 23.92 & 14.52 & 27.2 & 15.32 & 5.16 & 23.5 & 12.42 & 40.15 & 14.96 & 26.05\\ \hline 
 Tempr:1/3 &35.39 & 26.61 & 8.12 & 7.52 & 14.23 & 5.86 & 6.46 & 4.15 & 13.15 & 4.36 & 0.61 & 2.83 & 1.39 & 23.51 & 0.03 & 10.28\\ \hline 
  Tempr:1/4 &
15.22 & 7.26 & 10.83 & 12.36 & 3.3 & 10.43 & 11.97 & 8.82 & 2.78 & 9.57 & 6.2 & 18.11 & 16.8 & 5.46 & 14.95& 10.27 \\  \hline 
  % Tempr:1/5 & 3.42 & 10.67 & 20.6 & 30.3 & 18.48 & 27.85 & 30.49 & 24.98 & 19.23 & 26.46 & 17.14 & 36.07 & 33.3 & 10.33 & 31.77 & 22.74 \\  \hline 
 \multicolumn{17} {|c|}{Normal Distribution. First: Per-class covariance; next: cov based on the whole dset}\\  \hline 
PerClsCov & -54.11 & -47.97 & -53.49 & -33.17 & -43.14 & -23.86 & -27.9 & -17.88 & -29.68 & -16.82 & -6.29 & -30.61 & -19.15 & -42.52 & -22.08 &
31.24 \\ \hline
PerDsetCov & -40.41 & -49.58 & -33.95 & -18.44 & -38.05 & -25.92 & -24.33 & -9.0 & -27.69 & -8.31 & -6.2 & -17.37 & -15.19 & -48.43 & -15.13 &
25.2 \\ \hline

CovNoMean & -46.42 & -45.12 & -30.04 & -15.89 & -28.38 & -14.35 & -21.47 & -10.21 & -26.73 & -10.78 & 0.06 & -30.13 & -16.51 & -38.62 & -12.28 &
23.13 \\ \hline



Cov Bias & -34.83 & -45.4 & -33.89 & -18.45 & -38.05 & -25.9 & -24.34 & -9.01 & -27.51 & -8.37 & -6.2 & -17.35 & -15.22 & -46.78 & -15.11 &
24.42 \\ \hline

PerClsScale &-30.21 & -45.09 & -31.22 & -17.95 & -30.22 & -24.67 & -20.97 & -9.03 & -25.58 & -8.17 & -6.15 & -14.65 & -14.91 & -42.48 & -14.55 &
22.39 \\ \hline
 \multicolumn{17} {|c|}{Per Batch Scale: Apply logsumexp across batch dimention }\\  \hline 

BSize 32&-17.03 & -14.65 & -22.35 & 0.5 & 0.96 & 6.15 & 3.09 & 6.71 & 1.4 & 8.99 & 8.44 & 1.97 & 10.25 & -18.33 & 9.68 & 8.7
\\ \hline

BSize 64& -18.23 & -17.1 & -21.2 & -1.45 & -1.82 & 2.32 & 1.54 & 1.58 & -5.39 & 5.4 & 4.99 & -2.28 & 5.57 & -21.58 & 6.55 & 
7.8 \\ \hline

CovNoMean & -25.57 & -21.86 & -31.53 & -11.65 & -22.63 & -4.55 & -8.92 & 1.44 & 0.66 & 4.34 & 15.12 & -10.17 & -2.82 & -16.44 & -4.52 &
12.14\\ \hline

BSize 128 &  -17.95 & -17.81 & -18.64 & -1.86 & -3.97 & 1.21 & 0.23 & -1.31 & -9.96 & 3.61 & 3.87 & -3.89 & 3.25 & -24.58 & 3.25 &7.69\\ \hline

\multicolumn{17} {|c|}{Use Updated GT accuracy for calculating MAE}\\  \hline 
BSize 32 &-1.04 & -0.83 & -15.04 & 10.16 & 9.53 & 12.8 & 12.49 & 7.54 & 10.22 & 13.3 & 7.34 & 10.87 & 11.19 & -3.65 & 9.81 & 9.0\\ \hline

BSize 128 & -2.3 & -3.68 & -11.07 & 8.4 & 5.28 & 8.14 & 9.73 & 0.98 & -1.27 & 7.99 & 3.99 & 5.07 & 5.64 & -10.71 & 4.25 & 5.9\\ \hline

\multicolumn{17} {|c|}{Softmax with LogSum trick}\\  \hline 
BSize 64 & -2.6 & -3.03 & -2.93 & -4.69 & -2.41 & -4.02 & -3.05 & -7.41 & -14.04 & -5.09 & -3.39 & -3.36 & -4.1 & 3.64 & -5.62 & 4.62 \\
%\multicolumn{17} {|c|}{Consider the prediction incorrect if there is at least one gradient to 1/k that is smaller than the original }\\  \hline 
%k=2 & -56.11 & -48.06 & -44.88 & -29.85 & -36.72 & -22.64 & -26.49 & -15.53 & -28.93 & -16.69 & -5.17 & -27.89 & -14.7 & -42.39 & -17.83 & 28.92\\  \hline 

%\multicolumn{17} {|c|}{Consider the prediction incorrect if the  gradient to 1/(num of classes) is smaller than the gradient wrt 1/k. \textit{All predictions are larger than 95\%}}\\  \hline 
%k=2 & -72.27 & -65.57 & -72.41 & -46.79 & -54.11 & -34.6 & -41.82 & -24.98 & -41.19 & -25.96 & -9.27 & -46.38 & -26.37 & -58.35 & -30.18 & 43.34 \\ \hline

%\multicolumn{17} {|c|}{Per-sample gradient alignment: Per-sample gradient to mean gradient of that class (overestimates: most predictions - over 80\%)}\\  \hline 
%Weight & 63.66 & 56.33 & 55.29 & 36.42 & 43.04 & 27.51 & 32.55 & 19.17 & 34.21 & 20.53 & 7.12 & 35.67 & 19.15 & 49.66 & 22.18 & 34.83 \\ \hline 

%\multicolumn{17} {|c|}{Temperature based on the average gradient: Average Cosine distance with vs without updating Batch Norm Mean and Var}\\  \hline 
%Cos & 29.51 & 18.1 & \color{red} 27.08 & 21.72 & 27.26 & 11.52 & 28.54 & 1.32 & 15.27 & 18.43 & 6.35 & 16.11 & 17.47 & 2.88 & 7.32 & 16.59 \\ \hline 
%Manh & 8.43 & 14.69 & 26.25 & 8.91 & 21.5 & 17.71 & 22.53 & {\color{red} 14.11} & {\color{red} 22.4} & 15.31 & 6.97 & 8.6 & 12.96 &  {\color{red} 30.77} & {\color{red}10.36} & 16.10 \\ \hline 

%\multicolumn{17} {|c|}{Temperature based on the tightness of the classes (mean pairwise Euclidean distance within classes)}\\  \hline 
%Mean &28.2 & 17.48 & 1.04 & 5.2 & 1.84 & 4.56 & 5.14 & 8.14 & 1.57 & 3.2 & 2.14 & 0.02 & 13.68 & 10.52 & 13.22 &
%\textbf{7.72} \\ \hline 
%Median & 29.04 & 18.17 & 0.17 & 5.06 & 2.0 & 4.6 & 5.04 & 8.23 & 1.65 & 3.09 & 1.7 & 0.49 & 13.86 & 10.78 & 13.22 & \textbf{7.80}\\ \hline
%Mean$_{rnd}$ & 29.65 & 19.36 & 2.89 & 4.04 & 3.3 & 2.09 & 3.51 & 8.82 & 0.8 & 4.0 & 1.88 & 2.83 & 15.53 & 11.04 & 14.95 &
%8.31 \\ \hline
% Median$_{rnd}$ & 29.65 & 20.48 & 6.18 & 4.04 & 3.3 & 2.09 & 3.51 & 8.82 & 0.8 & 4.0 & 1.88 & 2.83 & 15.53 & 11.04 & 14.95 & 8.60 \\ \hline
  &   &   &   &   &   &   &   &   &   &   &   &   &   &  & & \\\
GT Acc &  27.67 & 34.29 & 27.08 & 53.06 & 45.68 & 65.25 & 57.98 & 74.93 & 58.7 & 73.99 & 90.7 & 53.31 & 73.41 & 41.55 & 69.7 & 56.48 \\ \hline

GT BSize 32 & 43.66 & 48.11 & 34.39 & 62.72 & 54.25 & 71.9 & 67.38 & 75.76 & 67.52 & 78.3 & 89.6 & 62.21 & 74.35 & 56.23 & 69.83 & 63.74 \\ \hline
GT BSize 128 &43.32 & 48.42 & 34.65 & 63.32 & 54.93 & 72.18 & 67.48 & 77.22 & 67.39 & 78.37 & 90.82 & 62.27 & 75.8 & 55.42 & 70.7  & 64.15\\ \hline
\bottomrule
\end{tabular}
}
}
\end{center}
\vspace{-1ex}
\end{table*}






\begin{table*}[ht]

\begin{center}
\caption{Mean Absolute Error Between Predicted and Ground Truth Accuracy for \textbf{Digits, DomainNet and Cifar10.1}}
%\vspace{-2ex}
\label{table:layer_choice}
\hspace*{-9ex} \scalebox{0.9}{
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{|l|c|c|c|c||c|c|c|c|c|c|c||c||c|c|c|c|}

\toprule
%\hline

% ToDo: Katya Left indent 

 % &\multicolumn{4}{|c|}{ Digits, MiniVGG} &\multicolumn{4}{|c|}{COCO, AlexNet}\\
 
% & \multicolumn{4}{|c|}{Size = 1000}\\

 & USPS & SVHN & SYNTH &\textbf{ Mean  }& ClipArt & Infographic & Painting & QuickDraw & Photo & Sketch & \textbf{Mean} & CIFAR10.1 \\\hline
 
 \multicolumn{17} {|c|}{Baselines} \\ \hline
   Probab & 5.53 & 35.44 & 13.26 & 18.07 & 
   &&&&&&&
   -2.2
    \\ \hline
Bias (to rand) &6.98 & 35.97 & 14.6 &
19.18   
&&&&&&&&
-2.1
   \\ \hline

%Bias (to one-hot) &-18.54 & -58.41 & -49.34&
%42.09
%&&&&&&&&
%-7.8
%   \\ \hline
  Entropy & 12.36 & 37.7 & 19.87 & 23.30
  &&&&&&&&
  0.2
  \\ \hline
OOD Loss & 49.83 & 40.75 & 33.9 & 41.48
&&&&&&&&
-2.1
\\ \hline
 
 
 \multicolumn{17} {|c|}{Norm Distribution: 1- Cov for all classes; 2- Biased Cov}\\  \hline 
Cov & -6.28 & 2.39 & -6.7 & 5.12 &
&&&&&&& -5.65 & \\ \hline
Cov Bias & -6.28 & 2.16 & -6.72 & 
5.05 &&&&&&& & \\ \hline
CovPerClScale &-3.39 & 8.7 & -0.61&4.23
&&&&&&&  &
 \\ \hline
CovPerClScaleBias &-3.39 & 8.7 & -0.61&4.23
&&&&&&&  &
 \\ \hline

 \multicolumn{17} {|c|}{Per Batch Scale: Apply logsumexp across batch dimention }\\  \hline 

BSize 32 &-3.84 & 6.53 & -3.17 & 4.51 &
&&&&&&&  &
 \\ \hline
BSize 64 &-5.48 & 7.61 & -1.73 & 4.94 &
4.64 & \textbf{-34.69} & 0.84 &\textbf{-62.16} &9.22&1.87 &
&&&&  &
 \\ \hline

 BSize 512 &-7.97 & 8.34 & -0.49 & 5.59 &
&&&&&&&  &
 \\ \hline

 \multicolumn{17} {|c|}{Softmax with LogSumExp Trick}\\  \hline 
 BSize 64 & 19.03 & 31.9 & 22.82 & 24.58 \\ \hline
BSize 512 & 14.5 & 34.15 & 17.05 & 21.90 \\ \hline

 \multicolumn{17} {|c|}{Use Updated GT accuracy for calculating MAE}\\  \hline 
 BSsize 32 & -4.33 & 3.27 & -4.12 & 3.90& 
&&&&&&&  &  \\ \hline
 BSsize 64 & -3.79 & 4.91 & -2.41 & 3.70& 
&&&&&&&  &  \\ \hline

  BSsize 512 &-4.73 & 6.05 & -0.57 & 3.78 &
&&&&&&&  &
 \\ \hline
 
 \multicolumn{17} {|c|}{Fixed Temperature}\\  \hline 
 No Temp & -7.82 & 27.3 & -7.45 & 14.19 &
 -2.79 & -2.39 & -7.3 & -17.6 & -6.87 & -8.76& 7.61 &
 -10.0 & 
 \\ \hline
 Tempr:1.1 & -9.52 & 24.83 & -10.9 & 15.08 
 & -7.08 & -7.17 & -12.25 & -24.16 & -11.27 & -13.61 & 12.58
 &-10.35
 \\ \hline
 Tempr:0.9 & -6.03 & 29.71 & -3.12 & 12.95
 & 2.06 & 2.07 & -1.8 & -10.72 & -1.73 & -3.48 & 3.64
& -9.7
 \\ \hline
 Tempr:0.8 & -3.54 & 32.1 & 1.97 & 12.53 
 & 7.89 & 6.17 & 4.45 & -3.84 & 4.34 & 2.76 &4.91
&-9.25
\\ \hline
 Tempr:0.7 & -0.2 & 34.32 & 7.83 & 14.11 &
 14.85 & 9.71 & 11.47 & 2.46 & 11.72 & 9.81 &
10.00 
& -8.9
\\ \hline
 
 Tempr:0.3 &57.05 & 41.01 & 38.27 &45.44 &
54.48 & 19.64 & 42.59 & 12.62 & 53.37 & 44.94
& 37.94
& 1.3
\\ \hline

%\multicolumn{17} {|c|}{Temperature based on the tightness of the classes (mean pairwise Euclidean distance within classes)}\\  \hline 
%Mean &81.46 & 41.56 & 50.66 &
%57.89  &  58.21 & 19.92 & 45.81 & 12.64 & 58.36 & 47.97 & 40.48 & \textbf{3.85} \\ \hline 
%Median & 81.46 & 41.48 & 50.66 & 57.86 &
%58.21 & 19.92 & 45.81 & 12.64 & 58.36 & 47.97 & 40.48 & \textbf{3.7} \\ \hline
%Mean$_{rnd}$ & 29.65 & 19.36 & 2.89 & 4.04 & 3.3 & 2.09 & 3.51 & 8.82 & 0.8 & 4.0 & 1.88 & 2.83 & 15.53 & 11.04 & 14.95 &
%8.31 \\ \hline
% Median$_{rnd}$ & 29.65 & 20.48 & 6.18 & 4.04 & 3.3 & 2.09 & 3.51 & 8.82 & 0.8 & 4.0 & 1.88 & 2.83 & 15.53 & 11.04 & 14.95 & 8.60 \\ \hline
  &   &   &   &   &   &   &   &   &   &   &   &   &   &  & & \\\hline
GT Acc & 81.46 & 41.59 & 50.66 & 57.90 &
58.21 & 19.92 & 45.81 & 12.64 & 58.36 & 47.97 & &
88.25
\\ \hline
GT Acc BS 32& 80.97 & 38.33 & 49.71 & 56.33&
&  &  & &  &  & & \\ \hline
GT Acc BS 64&  83.16 & 38.89 & 49.98 & 57.34 &
1.77 & 16.86  & 25.93 &0.96&32.53 & 27.61
  &  & & \\ \hline
GT Acc BS 256& 84.7 & 39.29 & 50.59 & 58.19&
&  &  & &  &  & & \\ \hline
\bottomrule
\end{tabular}
}
}
\end{center}
\vspace{-1ex}
\end{table*}




\begin{table*}[ht]

\begin{center}
\caption{Mean Absolute Error Between Predicted and Ground Truth Accuracy for \textbf{ImageNet-Corrupted.} \textbf{Source-Free}}
%\vspace{-2ex}
\label{table:layer_choice}
\hspace*{-9ex}\scalebox{0.8}{
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\toprule
%\hline

% ToDo: Katya Left indent 

 % &\multicolumn{4}{|c|}{ Digits, MiniVGG} &\multicolumn{4}{|c|}{COCO, AlexNet}\\
 
% & \multicolumn{4}{|c|}{Size = 1000}\\
  \hline
 & gauss & shot & impls  & defoc & glass  &motion  & zoom  & snow & frost & fog & bright& contr & elast &  pix & jpg &speck &gblur &spat & sat & Mean \\\hline
 \multicolumn{21} {|c|}{Fixed Temperature. }\\  \hline 
 No Temp & 6.14 & 5.47 & 5.02 & 4.79 & 1.38 & 2.16 & 1.74 & 13.0 & 2.63 & 5.9 & 2.01 & 1.3 & 13.35 & 0.63 & 1.0 & 6.58 & 3.42 & 16.21 & 1.02 &
4.93\\ \hline

 Tempr:0.9 &3.18 & 2.22 & 2.19 & 3.02 & 3.58 & 4.6 & 3.28 & 7.05 & 2.12 & 0.31 & 7.99 & 1.99 & 6.64 & 4.7 & 6.39 & 1.71 & 4.8 & 8.44 & 5.15&
4.17\\ \hline
 Tempr:0.8 &0.94 & 0.03 & 0.12 & 1.69 & 5.22 & 6.59 & 7.95 & 1.56 & 6.43 & 4.54 & 14.64 & 2.39 & 0.1 & 9.84 & 11.86 & 2.32 & 5.8 & 0.59 & 11.57&
4.95\\ \hline


Tempr:1/2 &1.62 & 2.46 & 1.93 & 0.26 & 7.35 & 9.84 & 16.87 & 9.31 & 14.05 & 12.57 & 38.96 & 2.75 & 13.2 & 21.33 & 26.03 & 8.37 & 7.08 & 17.53 & 31.91 &
12.81\\ \hline
Tempr:1/3 & 1.67 & 2.56 & 1.96 & 0.35 & 7.48 & 10.12 & 18.0 & 10.29 & 14.85 & 13.38 & 48.08 & 2.75 & 14.42 & 23.2 & 29.13 & 8.84 & 7.13 & 19.93 & 38.79&
14.36 \\ \hline
Tempr:1/4 & 1.67 & 2.56 & 1.96 & 0.35 & 7.48 & 10.12 & 18.02 & 10.29 & 14.87 & 13.41 & 48.75 & 2.75 & 14.45 & 23.3 & 29.26 & 8.85 & 7.13 & 20.01 & 39.32 &
14.45\\ \hline


\multicolumn{21} {|c|}{Temperature based on the tightness of the classes (mean pairwise Euclidean distance within classes)}\\  \hline 
Mean &1.67 & 2.56 & 1.96 & 0.35 & 7.48 & 10.12 & 18.03 & 10.29 & 14.87 & 13.41 & 48.77 & 2.75 & 14.45 & 23.3 & 29.27 & 8.85 & 7.13 & 20.01 & 39.35 &
14.45 \\ \hline 
Median &1.67 & 2.56 & 1.96 & 0.35 & 7.48 & 10.12 & 18.03 & 10.29 & 14.87 & 13.41 & 48.77 & 2.75 & 14.45 & 23.3 & 29.27 & 8.85 & 7.13 & 20.01 & 39.35 &
14.45 \\ \hline 

  &   &   &   &   &   &   &   &   &   &   &   &   &   &  & & &&&&\\\
  Acc-10 &8.65 & 11.11 & 10.02 & 3.17 & 24.41 & 30.2 & 44.58 & 31.44 & 38.94 & 37.66 & 81.0 & 12.4 & 39.76 & 54.27 & 61.44 & 28.02 & 24.66 & 49.06 & 71.62 & \\ \hline
GT Acc &1.67 & 2.56 & 1.96 & 0.35 & 7.48 & 10.12 & 18.03 & 10.29 & 14.87 & 13.41 & 48.77 & 2.75 & 14.45 & 23.3 & 29.27 & 8.85 & 7.13 & 20.01 & 39.35 & \\ \hline



\bottomrule
\end{tabular}
}
}
\end{center}
\vspace{-1ex}
\end{table*}

([0.8, 0.1, 0.0, 0.0] - [1, 0, 0, 0])*X

([0.8, 0.1, 0.0, 0.0] - [1/4, 1/4, 1/4, 1/4])*X


\begin{table*}[ht]

\begin{center}
\caption{Mean Absolute Error Between Predicted and Ground Truth Accuracy for \textbf{ImageNet-Corrupted, WideResNet} \textbf{Source-Free}}
%\vspace{-2ex}
\label{table:layer_choice}
\hspace*{-9ex}\scalebox{0.75}{
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\toprule
%\hline

% ToDo: Katya Left indent 

 % &\multicolumn{4}{|c|}{ Digits, MiniVGG} &\multicolumn{4}{|c|}{COCO, AlexNet}\\
 
% & \multicolumn{4}{|c|}{Size = 1000}\\
  \hline
 & gauss & shot & impls  & defoc & glass  &motion  & zoom  & snow & frost & fog & bright& contr & elast &  pix & jpg &speck &gblur &spat & sat & Mean \\\hline
 \multicolumn{21} {|c|}{Fixed Temperature. Values: GT - Prediction; (negative=overestimation; positive=underestimation) }\\  \hline 
 %No Temp &6.42 & 2.87 & 7.81 & 4.4 & 5.52 & 6.61 & 9.56 & 8.35 & 7.81 & 0.35 & 9.4 & 0.41 & 11.85 & 12.83 & 10.75 & 1.73 & 4.03 & 2.42 & 2.36 
 %& 6.08\\ \hline

 No Temp &-6.42 & -2.87 & -7.81 & -4.4 & 5.52 & 6.61 & 9.56 & 8.35 & 7.81 & 0.35 & 9.4 & 0.41 & 11.85 & 12.83 & 10.75 & 1.73 & 4.03 & 2.42 & 2.36 &
6.08 \\ \hline
 

Energy &-6.15 & -5.48 & -5.02 & -4.79 & 1.37 & 2.14 & -1.78 & -13.04 & -2.65 & -5.94 & 1.97 & 1.29 & -13.39 & -0.66 & 0.96 & -6.61 & 3.42 & -16.26 & -1.06
& 4.94\\ \hline
\multicolumn{21} {|c|}{Consider the prediction incorrect if the  gradient to 1/k is smaller than the gradient wrt one-hot encoding.  }\\  \hline 

k=3 &
-2.65 & 0.31 & -3.78 & -3.3 & 7.9 & 8.44 & 13.19 & 11.7 & 10.08 & 0.47 & 16.77 & 0.41 & 18.51 & 20.78 & 20.04 & 6.27 & 4.89 & 8.02 & 10.4 &
8.83 \\ \hline 

k=5 & -4.07 & -0.91 & -5.28 & -3.75 & 6.93 & 7.72 & 11.62 & 10.28 & 9.12 & 0.42 & 13.59 & 0.41 & 15.51 & 17.16 & 15.73 & 4.45 & 4.53 & 5.55 & 6.87 &
7.57 \\ \hline

k=10 & -4.93 & -1.67 & -6.22 & -3.98 & 6.35 & 7.27 & 10.76 & 9.54 & 8.62 & 0.4 & 11.85 & 0.41 & 13.99 & 15.4 & 13.52 & 3.43 & 4.35 & 4.29 & 5.12 &
6.95 \\ \hline

\multicolumn{21} {|c|}{Consider the prediction incorrect if the  gradient to 1/(num of classes) is smaller than the gradient wrt 1/k.}\\  \hline 

k=2 & -16.64 & -11.02 & -18.44 & -6.99 & 0.5 & 2.78 & 2.89 & 1.76 & 3.05 & 0.18 & -2.78 & 0.39 & 0.88 & 0.7 & -2.57 & -8.59 & 1.92 & -7.98 & -11.33 &
5.33 \\ \hline

k=3 &-26.05 & -18.76 & -27.97 & -8.84 & -2.75 & 0.07 & -1.15 & -2.39 & -0.59 & -0.03 & -9.42 & 0.39 & -5.26 & -5.3 & -8.43 & -17.12 & 0.41 & -14.59 & -19.42 &
8.89 \\ \hline

k=5 & -43.78 & -33.64 & -45.39 & -11.64 & -7.35 & -3.88 & -6.66 & -8.17 & -6.68 & -0.38 & -17.61 & 0.31 & -13.13 & -12.6 & -14.96 & -31.41 & -1.95 & -24.14 & -29.87 &
16.50 \\ \hline

\multicolumn{21} {|c|}{Temperature based on the tightness of the classes (mean pairwise Euclidean distance within classes)}\\  \hline 
Mean &4.53 & 7.14 & 3.48 & 0.32 & 15.56 & 14.48 & 24.68 & 21.86 & 17.08 & 0.72 & 43.03 & 0.42 & 42.07 & 49.96 & 57.46 & 18.86 & 7.87 & 26.95 & 34.68 &
20.58 \\ \hline 
Median &4.53 & 7.14 & 3.48 & 0.32 & 15.56 & 14.48 & 24.68 & 21.86 & 17.08 & 0.72 & 43.03 & 0.42 & 42.07 & 49.96 & 57.46 & 18.86 & 7.87 & 26.95 & 34.68 &
20.58 \\ \hline 

  &   &   &   &   &   &   &   &   &   &   &   &   &   &  & & &&&&\\\
  Acc-10 &13.96 & 18.84 & 11.82 & 2.97 & 39.37 & 37.09 & 52.98 & 47.42 & 39.02 & 3.64 & 74.18 & 2.99 & 71.32 & 79.67 & 85.23 & 39.39 & 23.67 & 54.72 & 64.58 & \\ \hline
GT Acc &4.53 & 7.14 & 3.48 & 0.32 & 15.56 & 14.48 & 24.68 & 21.86 & 17.08 & 0.72 & 40.66 & 0.42 & 42.07 & 49.96 & 57.46 & 18.86 & 7.87 & 26.95 & 34.68 & \\ \hline



\bottomrule
\end{tabular}
}
}
\end{center}
\vspace{-1ex}
\end{table*}


\begin{table*}[ht]

\begin{center}
\caption{Mean Absolute Error Between Predicted and Ground Truth Accuracy for CIFAR-Corrupted. \textbf{The threshold is mined}}
%\vspace{-2ex}
\label{table:layer_choice}
\scalebox{0.9}{
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\toprule
%\hline

% ToDo: Katya Left indent 

 % &\multicolumn{4}{|c|}{ Digits, MiniVGG} &\multicolumn{4}{|c|}{COCO, AlexNet}\\
 
% & \multicolumn{4}{|c|}{Size = 1000}\\
  \hline
 & gauss & shot & impls  & defoc & glass  &motion  & zoom  & snow & frost & fog & bright& contr & elast.&  pix & jpg & Mean \\\hline
 Probab &26.58 & 19.14 & 4.59 & 1.48 & 8.79 & 0.23 & 0.67 & 1.6 & 6.71 & 1.66 & 2.59 & 2.6 & 6.77 & 14.86 & 5.0 & 6.88 \\ \hline 
\textbf{Bias } & 26.32 & 18.97 & 4.36 & 1.21 & 8.61 & 0.04 & 0.45 & 1.71 & 6.47 & 1.85 & 2.65 & 2.86 & 6.95 & 14.63 & 5.2 & 6.82\\ \hline
Entropy & 25.69 & 17.99 & 2.97 & 0.43 & 7.98 & 0.47 & 0.35 & 2.08 & 6.03 & 2.33 & 2.84 & 3.66 & 7.4 & 13.95 & 5.75 & 6.66  \\ \hline 
OOD loss & 30.03 & 20.18 & 2.92 & 7.24 & 2.71 & 4.14 & 5.39 & 2.02 & 8.03 & 2.97 & 3.16 & 13.49 & 11.15 & 16.55 & 9.96 & 9.33\\ \hline
  &   &   &   &   &   &   &   &   &   &   &   &   &   &  & & \\\
GT Acc &  27.67 & 34.29 & 27.08 & 53.06 & 45.68 & 65.25 & 57.98 & 74.93 & 58.7 & 73.99 & 90.7 & 53.31 & 73.41 & 41.55 & 69.7 & \\ \hline

\bottomrule
\end{tabular}
}
}
\end{center}
\vspace{-1ex}
\end{table*}



\newpage
\begin{table*}[ht]

\begin{center}
\caption{Mean Absolute Error Between Predicted and Ground Truth Accuracy for CIFAR-Corrupted. \textbf{Source-Free, BN Enabled}}
%\vspace{-2ex}
\label{table:layer_choice}
\scalebox{0.9}{
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\toprule
%\hline

% ToDo: Katya Left indent 

 % &\multicolumn{4}{|c|}{ Digits, MiniVGG} &\multicolumn{4}{|c|}{COCO, AlexNet}\\
 
% & \multicolumn{4}{|c|}{Size = 1000}\\
  \hline
 & gauss & shot & impls  & defoc & glass  &motion  & zoom  & snow & frost & fog & bright& contr & elast.&  pix & jpg & Mean \\\hline
 \multicolumn{17} {|c|}{Fixed Temperature. Overestimates: all the predictions- over 92\%}\\  \hline 
 No Temp & 23.65 & 21.76 & 30.06 & 11.18 & 28.8 & 12.13 & 10.85 & 15.34 & 14.8 & 13.37 & 7.68 & 9.62 & 19.9 & 16.71 & 22.9 & 17.25 \\ \hline
  &   &   &   &   &   &   &   &   &   &   &   &   &   &  & & \\\
GT Acc & 70.69 & 72.82 & 62.66 & 86.01 & 63.88 & 84.71 & 86.48 & 81.11 & 81.25 & 83.4 & 90.42 & 85.91 & 74.97 & 79.01 & 71.35 & \\ \hline
\bottomrule
\end{tabular}
}
}
\end{center}
\vspace{-1ex}
\end{table*}




Currently, we consider the following approach: given an image, calculate the Cross Entropy Loss w.r.t. each label. Backpropogate the loss for the resulting batch; take the mean of the bias gradient in the last FC layer. The final value is the norm of the gradient mean.

Bias depends only on the activation of that layer, and not the gradients of the deeper layers. 
Assume $z = W X + b $  - the last fully connected layer of the network; $s = softmax(z)$
$$\frac{\partial L} {\partial b_i}  = \frac{\partial L} {\partial z_i} = s_i - y_i $$

For the batch, constructed as described above, the mean of the gradient becomes: 
$$ \frac{1}{C} \sum_{i=0}^C  \frac{\partial L} {\partial b} = \frac{s_i - 1 + s_i(n-1)}{n} = s_i - \frac{1}{n}$$

The final metric: 
$$ || \frac{1}{C} \sum_{i=0}^C \frac{\partial L_j} {\partial b} || = || s - \frac{1}{n}||$$

Similarly, we can express the mean of the gradients of W:
$$ mean ( \frac{\partial L} {\partial W} )= ( s - \frac{1}{n}) X $$


Similarly, we can express the variance of the gradients of W:
$$ variance (\frac{\partial L} {\partial W}) =  \frac{1}{n(s-1)} X^T $$



